Characterizing Issue Management in Runtime Systems

Modern programming languages like Java require runtime systems to support the implementation and deployment of software applications in diverse computing platforms and operating systems. These runtime systems are normally developed in GitHub-hosted repositories based on close collaboration between large software companies (e.g., IBM, Microsoft) and OSS developers. However, despite their popularity and broad usage; to the best of our knowledge, these repositories have never been studied. We report an empirical study of around 118K issues from 34 runtime system repos in GitHub. We found that issues regarding enhancement, test failure and bug are mostly posted on runtime system repositories and solution related discussion are mostly present on issue discussion. 82.69% issues in the runtime system repositories have been resolved and 0.69% issues are ignored; median of issue close rate, ignore rate and addressing time in these repositories are 76.1%, 2.2% and 58 days respectively. 82.65% issues are tagged with labels while only 28.30% issues have designated assignees and 90.65% issues contain at least one comment; also presence of these features in an issue report can affect issue closure. Based on the findings, we offer six recommendat

==> Dashboard.tex <==
\section{A Dashboard for Information Type Summarization} \label{sec:dashboard}
In order to assist the project stakeholders of open source software systems and our industrial partner, IBM; we have summarized our findings of issue discussion analysis and deployed as a chrome extension tool. This tool is easy to use and works on github start page of a project. It displays two things: \begin{inparaenum}[(1)] \item the distribution of information types of issue discussions of a project in a pie chart and \item the evolution of information types over the year from beginning of the project to current date with multiple line charts \end{inparaenum}. Tooltip of each slice of the pie chart shows the total number of information type along with name of the information type; same for each point in the line chart. Legend maps between the color and name of information type and the current percentage of the distribution. Fig. \ref{fig:snippet} shows a snippet of the tool at the start page of the github. User can select to display the data about all, open or closed issues using the button displayed above. 
\begin{figure}[t]
%\centering
%\hspace{-1cm}
\includegraphics[scale=0.5]{Images/tool.pdf}
\caption{Issue Analytic chrome extension tool}
\label{fig:snippet}
%\vspace{-.5cm}
\end{figure}

==> Model.tex <==
\section{Automatic Detection of Information Types} This section answers the first research question of developing a information type classifier that beats the state-of the art model. 
\subsection{Can we improve the detection performance of the information types in issue reports? (RQ1)} 
\subsubsection{Motivation} It can be difficult to retrieve information from a lengthy and complex issue discussion. Therefore, an automated classifier is required to label the discussion in mass level that can more accurately identify each information type from issue discussion. Though to automatically identify the information types from issue discussion, Arya et al. \cite{InfoTypesOSSDiscussion} developed several ML classifiers; where their random forest classifier using conversational features performs the best with 61\% weighted f1-score; the classification accuracy can be improved. Therefore, we approached to develop another ML model that can outperform the previous one.
\subsubsection{Approach}
 To train their model,  Arya et al. \cite{InfoTypesOSSDiscussion} prepared a dataset which consists 15 complex and lengthy issues collected from three Github hosted Artificial Intelligence (AI) libraries; namely, TensorFlow, scikit-learn, spaCy and  has total 4330 sentences containing 13 information types. Then they extracted 14 conversational features about the position of a sentence in a comment or thread, relative posting time with respect to beginning or ending comment and previous or next comment, original and respective length with comment or thread,  the author's association with repository, existence of code and whether comment poster is the poster of the issue. We have reused this dataset and used 5 fold cross-validation approach for obtaining the result. For comparison, we considered Arya's et al. \cite{InfoTypesOSSDiscussion} model as our baseline.
\subsubsection{Result}
 We succeeded to develop a lightGBM \cite{lightgbm} classifier using the same conversational features extracted by Arya et al. \cite{InfoTypesOSSDiscussion}  and our model outperforms the baseline model by achieving 64\% weighted f1-score. The developed model also gives more f1-score on 11 classes while baseline model outperforms in detecting only Contribution and Commitment and Bug Reproduction class. The performance of the both models are listed in table \ref{tab:dataset_perf} for comparison.

\begin{table}[!ht]
        \caption{Performace of lightGBM and baseline classifier for automatic detection of information types of issue discussion (Pr = Precision, Rc = Recall, F1 = F1-score)}
    \label{tab:dataset_perf}
\begin{adjustbox}{width=\columnwidth}
    \centering

    \begin{tabular}{l|l|l|l|l|l|l|l}

    \toprule
         ~ & \multicolumn{2}{c}{\textbf{LightGBM}}& ~  & \multicolumn{3}{c}{\textbf{Baseline}} \\ 
        Label & Pr & Rc & F1  & Pr & Rc & F1  & Support \\ \midrule
        Action on Issue & 0.56 & 0.44 & \textbf{0.48} & 0.45 & 0.39 & 0.42 & 61 \\ 
        Bug Reproduction & 0.49 & 0.48 & 0.48 & 0.53 & 0.47 & \textbf{0.5} & 245 \\ 
        Contribution and Commitment & 0.29 & 0.14 & 0.19 & 0.25 & 0.19 & \textbf{0.21} & 83 \\ 
        Expected Behaviour & 0.41 & 0.38 & \textbf{0.39} & 0.42 & 0.28 & 0.33 & 124 \\ 
        Investigation and Exploration  & 0.65 & 0.64 & \textbf{0.64} & 0.6 & 0.65 & 0.62 & 377 \\
        Motivation & 0.57 & 0.53 & \textbf{0.55} & 0.56 & 0.53 & 0.54 & 288 \\ 
        Observed Bug Behaviour & 0.6 & 0.72 & \textbf{0.65} & 0.56 & 0.7 & 0.62 & 131 \\ 
        Potential New Issues and Requests & 0.73 & 0.7 & \textbf{0.71} & 0.67 & 0.66 & 0.66 & 230 \\ 
        Social Conversation & 0.64 & 0.64 & \textbf{0.64} & 0.63 & 0.62 & 0.63 & 798 \\ 
        Solution Discussion & 0.71 & 0.75 & \textbf{0.73} & 0.68 & 0.71 & 0.69 & 1411 \\ 
        Task Progress & 0.31 & 0.15 & \textbf{0.2} & 0.27 & 0.14 & 0.18 & 125 \\ 
        Usage & 0.7 & 0.79 & \textbf{0.74} & 0.65 & 0.82 & 0.73 & 368 \\ 
        Workarounds & 0.69 & 0.52 & \textbf{0.59} & 0.58 & 0.45 & 0.49 & 89 \\ \midrule
        Weighted avg/total & 0.63 & 0.64 & \textbf{0.64} & 0.61 & 0.62 & 0.61 & 4330 \\ 
        \bottomrule
    \end{tabular}
\end{adjustbox}
\end{table}


\begin{tcolorbox}[flushleft upper, boxrule=1pt, arc=0pt, left=0pt, right=0pt, top=0pt, bottom=0pt, colback=white, after=\ignorespacesafterend\par\noindent]
\textbf{Summary of RQ1} Our developed ML classifier (lightGBM) outperformed the state-of-the-art model by achieving 64\% weighted f1-score. Also on class level, it beat the f1-score of 11 classes than the baseline model.
\end{tcolorbox}

\subsubsection{Misclassification Analysis} We further analyzed the reasons for misclassification of information types by the developed ML model. We find that there are two primary reasons for wrong classification. Firstly because the features related to the particular sentences were absent in the training set. This implies adding more accurate labelled data in the training set will improve the precision of detection. Another reason was sentences were labelled on the nature of its surrounding sentences or length. For example, a sentence of Solution Discussion type, 'The full individual binding wouldnt be too bad from my current starting point.', which is misclassified as Social Conversation since the sentence is tailed by the sentences of Social Conversation. 
%Also, we observed that using the text would be good indicator for information type detection since there are clearly presence of particular keywords in every information type. 


==> Motivation.tex <==
\section{Motivation} \label{sec:motivation}

\begin{comment}
\section{Motivation} \label{sec:motivation}
The information users or project maintainers are seeking for may or may not be present in issue discussion threads. However, they must spend a lot of time for reading through a great number of comments to be certain about it. In this situation, an automated information type identifier can come to the rescue by reducing the time and effort required for searching any specific information from issue discussions. There may be instances where project maintainers are looking for possible contributors but due to the in-depth conversation they missed the fact that someone had already shown interest in volunteering in the comment section. Or perhaps someone mentions a new bug or a feature request in the comment section rather than submitting a new issue. Similarly, before beginning to investigate a problem or while doing it, developers may want to have a look at the steps for reproducing the problem, the expected and observed bug behaviour, the findings of the investigation, any progress on the solution or any existing workaround. They also might have to spend a lot of time searching for pertinent comment for the similar reason. Again, users also sometimes want to know the solution progress or use a solution but if the discussion threads are long and complex, the entire procedure takes time. Fig. \ref{fig:examples} shows some example comments from issue discussion threads of Node project. In the first comment, participant shared that he missed the answer that was already give. Comment 2 and 3 talked about the existence of workaround that users might find helpful to work as a temporary solution for now. In comment 4, project maintainer wants to know the status or progress of the issue since the issue was without any recent comments for a long time and thus asking the community. All of these observations points out the necessity for finding proper information in a short time from a lengthy discussion. This observation has motivated us to look into this problem that can help project maintainers, developers, users or even researchers to find information quickly. Additionally, an empirical study will assist project maintainers to check the distribution of information present in their project's issue discussion threads and monitor the trend and evolution. Using this data, they can understand if they need to push for making any change in community guidelines.  
In order to recognize the information, Arya et al. \cite{InfoTypesOSSDiscussion} came up with a taxonomy of information types found on the issue discussion. Table \ref{tab:definition} lists down the definition of 13 information types that we will automatically classify. 


\begin{figure}[t]
\centering
%\hspace{-1cm}
\includegraphics[scale=0.4]{Images/examples.pdf}
\caption{Example comments from issue discussion thread of Node \#6456 where important comments are hidden in the midst of 173 comments}
\label{fig:examples}
\vspace{-.5cm}
\end{figure}

\begin{table}[!ht]
    \caption{Definition of information types found on issue discussion}
    \label{tab:definition}
\begin{adjustbox}{width=\columnwidth}
    \centering

    \begin{tabular}{l|p{50mm}|p{50mm}}
    \toprule
        \textbf{Information Type} & \textbf{Definition} & \textbf{Examples} \\ \midrule
        Action on Issue & Comments about actions perform for issue management like closing, reopening, labelling and others  & If no other comments, I think I'll just close this issue. \\ \hline
        Bug Reproduction & Any question, statement or report regarding the reproduction of the bug & I still cannot reproduce this issue. \\ \hline
        Contribution and Commitment & Comments about assigning or asking members for resolving an issue along with volunteer contribution or unwillingness & Yes, I'd like you to assign this to me. \\ \hline
        Expected Behaviour & The expected situation from user's perspective or personal preference and opinion & My suggestion/request in the near term would be to have an option to make the vocabulary read only so that users who want to be able to leave spacy alone to do streaming data processing don’t need to worry about changing memory requirements \\ \hline
        Investigation and Exploration & Suggesting investigation ideas or reporting results aout the cause of the issue  & This result confirms my hypothesis but also shows that the memory increase really isn’t all that significant... But it still points to a potential flaw in the design of the library. \\ \hline
        Motivation & Why an issue needs to resolved or a feature need to be added or changed & Right now, this method starves my GPU all the time, which is a shame because most other [deep learning] frameworks manage to make this much more performantly \\ \hline
        Observed Bug Behaviour & Questions or reports about the observed behaviour of a bug & I found strange behavior using the ‘pipe()’ method”, then started to describe this behavior \\ \hline
        Potential New Issues and Requests & Comments involving identifying new bugs or need of new features or any change while investigating an issue & As a side point, I note there seems to be a lot more joblib parallelisation overhead in master... that wasn’t there in 0.14. \\ \hline
        Social Conversation & Any kind of small talk or  showing gratitude or disappointment or other emotions.   & Thanks for your reply! \\ \hline
        Solution Discussion &  Suggestion or stament about design, implementation, constraints, challenges and references for solution & To alleviate this, I would suggest we define a Managed JNI interface to take it's place. \\ \hline
        Task Progress & Asking or providing update about the progress of the task towards the solution  & I am kind of stuck where this lookup for such a method could come from and how I could resolve that or work around the problem. \\ \hline
        Solution Usage &  Question or suggestion on how to use the new solution. & Please help me how to continue training the model [with the new release] \\ \hline
        Workarounds & Temporary solution before the official one & we may add `-Djava.security.manager=allow` for JDK18 as a temporary solution. \\ \bottomrule
    \end{tabular}
\end{adjustbox}
\end{table}

\begin{comment}\textbf{Runtime Systems.}
Most programming languages require the support of a framework to provide a platform on which programmes can be executed. This framework is known as a runtime system which  makes it possible for computer systems to run software programmes. For program execution and operation, runtime systems may play various roles like interacting with low level functions of memory management or high level functions of type checking. To execute the Java byte code, an engine is needed to provide the runtime environment, namely Java Virtual Machine (JVM).
\end{comment}
\end{comment}

==> Recommendation.tex <==
\section{Recommendation} \label{sec:reco}
The result of our empirical study shows issues are more likely to be closed when they have assignees. However only around 30\% issues have designated assignees. We recommend runtime system repository maintainers to use the assignee feature provided by GitHub for effective issue management. There are different tools that can be used for automated triaging \cite{AutomatedBugTriagingTopicModel,triagetoss,ImprovingBT,Li2021RevisitingTF, Zhang2017EnLDAAN,Kardoost2022DevRankerAE, Tao2017BugRE,Xi2018AnEA,Alazzam2020AutomaticBT}  and reduce manual work; maintainers can use these for this task. 
\begin{Recommendation}
 Runtime system project maintainers should assign issues to responsible experts as soon as an issue is reported. 
\end{Recommendation}

Again, we observed that having labels on the issues also affect the issue closure. Kim et al. \cite{multilabel} showed that projects that use multi-label features can manage issues more effectively.  Therefore, it is recommended to runtime system repository stakeholders to actively leverage this feature. They can use some automated issue labelling tools \cite{predictissuetype,tickettagger} for speeding up their work.

\begin{Recommendation}
 Runtime system project maintainers should tag issues with labels for effective issue management.
\end{Recommendation}

Apart from these, issue discussions also help an issue closure. Developers can be more clear of the issue from the reporter, discuss with their peers about issue investigation and  solution and can come up with a solution. Our result also shows, half of the discussion consists of only Solution Discussion. Therefore, we encouraged developers to actively engage on discussion if they find any trouble on understanding any issue and need help from peers and not hesitate or fear to ask.

\begin{Recommendation}
Developers should engage in discussion to be clear of the issues and discuss idea about investigation and solution. 
\end{Recommendation}


Again, descriptive and positive issue description can create a significant difference to the closure of the issue. We suggest issue reporters to explain all the details of the issue elaborately and provide all sorts of information. 

\begin{Recommendation}
Issue reporters should elaborately explain the issues.
\end{Recommendation}

Also, our result suggests presence of code can cause a significant difference to issue closure. Therefore, we would like to suggest issue reporters to add code blocks in markdown syntax for issues like bug, error or wrong output when available. This ways issue will be more precise and easy to understand for maintainers and developers.

\begin{Recommendation}
Issue reporters should add code snippets if available for describing an issue like bug, error or wrong output. 
\end{Recommendation}


From our analysis, we found that besides error, users often ask questions and request for enhancement. To address and reduce these issues, it is recommended to provide more clear instructions on how to use each function and strengthen documentations ; also share future plan of enhancement if possible. 

\begin{Recommendation}
Project maintainers should strengthen documentations and provide clear instructions of usage.
\end{Recommendation}


 
\begin{comment}
\section{Discussions} \label{sec:discussion}
In this study, we contributed in three categories; firstly we built an information type classifier, then using this, we conducted an empirical study of information types on runtime system issue reports and finally deployed an issue analytic tool as a chrome extension. All of this have potential to help  project stakeholders, e.g.: project managers, developers, users and triagers in various purposes. Additionally it can be highly valuable to the researchers to further conduct empirical study and and tool developers use the insights of the result in developing necessary tools. Enthusiasts or audiences of ITS can also get help from the issue analytic tool.

\subsection{Correlation between 13 information types}
First, we examine whether there is any association between the 13 information kinds in the empirical dataset we are studying. Since sentences of various information types are included in three groups of runtime system, it is possible that these types are interconnected and correlated. We used Spearman's correlation coefficient to assess the correlation between various information kinds obtained across the full dataset used for the empirical investigation in order to test the hypotheses. We report the Spearman’s coefficients between each pair of information types in fig. \ref{fig:spearman}. Some of the information types are positively correlated and some of them are negatively, we observe Contribution and commitment has strong positive correlations with 4 other information types (i.e. Action on Issue, Motivation, Potential New Issues and Requests and Workarounf ) with Spearman’s coefficients of +0.87. 

\begin{figure}[t]
\centering
%\hspace{-1cm}
\includegraphics[scale=0.4]{Images/infotype_spearman.pdf}
\caption{: Correlation between information type in three types of runtime system}
\label{fig:spearman}
%\vspace{-.5cm}
\end{figure}
\subsection{Implication of Issue Analytic Tool}
Audiences or project stakeholders can check the issue discussion trend of a project looking at the issue analytic tool along with the distribution of information types. Using this knowledge, project managers may provide guidelines to direct participants of the discussions to post only relevant and necessary comments to unclutter the space. This can be a indicator of a better project that can create a professional discussion space.

\subsection{Implication of study findings}  We discuss the implication of our study findings for the stakeholders below:

\textbf{Tool developers.}
Since this empirical study points out the topics that are mostly discussed in the issue threads, tool developers can leverage this information to identify the need of project stakeholders and design useful tools for the interested parties. Since discussion participants are mostly interested in the resolution process and half of the discussion is about Solution Discussion; summarizing the solution process and progress by identifying these comments can be a great opportunity for the tool developers. Also, there is a increasing trend of adding comments about Action on Issue and Task Progress on issue threads for better issue management; keeping that in mind, tool developers can focus on building more useful issue management tools to keep track of the actions and task progress of an issue. 

\textbf{Project stakeholders.} Project stakeholders can use the classifier to recognize the required information from issue discussion. They may further adopt this classifier for issue discussion navigation. 

\textbf{Researchers.} Researchers can use the information type classifier to conduct any large scale empirical research. Similar to issue discussion of github, this can be used in other platforms and applications or to examine other discussion threads like pull request discussions. 

\end{comment}

==> ThreatsToValidity.tex <==
\section{Threats to Validity}\label{subsec:validity}
\textbf{Internal validity} threats refer to the authors' biases while conducting a study. In order to mitigate the bias for manual labelling, we picked issues randomly for creating the sample dataset and picked at least one issue from each repository. By this way, we ensured that we do not select only certain types of issues and we do not discard any repositories no matter how small it is in terms of number of issues.  \textbf{Construct validity} threats refer to the error in data collection process.  To identify the runtime system projects, we used both topics and the project description metadata and followed best practices to analyze GitHub repositories. \textbf{External validity} threats concern the generalizability of the findings of this study. Since we are focusing on runtime system issues, we tried to gather as much as GitHub hosted runtime system projects and finally utilised 34 projects. To ensure significant amount of data and make our study generalizable as possible, we considered all issues for issue management analysis and for issue content analysis, we took a statistically significant sample to identify issue category and  information types of all sentences extracted from the issue threads. Our model can be applied to any similar platforms to get the empirical result about the issue addressing and management along with retrieving the distribution of information types in issue discussion.
\begin{comment}
\textbf{Internal validity} threats refer to the authors' biases while conducting a study. In order to mitigate the bias for developing the model, we used 10 fold cross-validation approach which divides the dataset in 10 equal parts; to every time use a single part for testing and others for training. By this way, it ensures not to share any data between train and test set and maintains the standard practices of evaluating a model. \textbf{Construct validity} threats refer to the error in data collection process. We used the same dataset developed and used by Arya et al. \cite{InfoTypesOSSDiscussion} that was prepared through exhaustive manual labelling by the authors. \textbf{External validity} threats concern the generalizability of the findings of this study. Since we are focusing on runtime system issues, we tried to gather as much as github hosted runtime system projects and finally utilised seven projects from three different groups. To ensure significant amount of data and make our study generalizable as possible, we considered all issues exist on the repositories with at least one comment and identified information types of all sentences extracted from the issue threads. Our model can be applied to any similar platforms to get the empirical result about the distribution of information types of issue discussion.
\end{comment}
